Understanding the Properties of Generated Corpora

Models for text generation have become focal for many research tasks and especially for the generation of sentence corpora. However, understanding the properties of an automatically generated text corpus remains challenging. We propose a set of tools that examine the properties of generated text corpora. Applying these tools on various generated corpora allowed us to gain new insights into the properties of the generative models. As part of our characterization process, we found remarkable differences in the corpora generated by two leading generative technologies.

==> fig_and_tables/datasets.tex <==
\begin{table}[h]
\centering
%  \def\arraystretch{2}
 \begin{tabular}{||c|c|c|c||} 
 \hline
 Name & Domain & Style & Size \\ [0.5ex] 
 \hline\hline
 Amazon & Phones & Reviews & 40k \\ \hline
News & Politics & News&30k \\ \hline
Yahoo & Health & Questions & 8.7k \\ \hline
\end{tabular}
\caption{Analysis of the Amazon, News and Yahoo! Answers corpora}
\label{tab:datasets}
\end{table}

==> fig_and_tables/generative_models.tex <==
\begin{table}
\small
\centering
\begin{tabular}{||c|M{1.7cm}|M{1cm}|M{1.2cm}|M{1.6cm}||}
\hline
Name & Type & Ext. Dataset & Training Phase & Generation input \\ \hline \hline
VAE & Autoencoder & - & +& Random\\ \hline
CVAE & Autoencoder & -&+& Random + Train sentence\\ \hline
MM & Markov Model & - & +&Random\\ \hline
GPT-2& Language Model & Web Pages & + & Train sentence\\ \hline
EDA & Rule-Based & Word-Net &- &Train sentence\\ \hline
\end{tabular}
\caption{Generation Models}
ֿ\label{tab:genmodel}
\end{table}

==> fig_and_tables/human_results.tex <==
\begin{table}
\small
\begin{tabular}{||M{1cm}|M{1.4cm}|M{1cm}|M{1.2cm}|M{1.2cm}||}
\hline
Model&Grammar& Make Sense & Domain Rel. & General\\
\hline \hline
Train&13.3&12&8.9&9.4\\
\hline
Test&13.3&11&8.3&8.7\\
\hline
VAE&\textbf{14}&\textbf{11.3}&\textbf{10.3}&\textbf{9.9}\\
\hline
CVAE&13.9&10&8.7&7.8\\
\hline
MM&11.2&5.3&6.2&4.6\\
\hline
GPT-2&11.6&5.8&6.4&5.4\\
\hline
EDA&8.8&4.3&6&3.6\\
\hline

\end{tabular}
\caption{Human Evaluation - Percentile of results ranked 4 or 5 from a 1-5 Likert scale}
\label{tab:human}
\end{table}

==> fig_and_tables/phone_results.tex <==
\begin{subtable}[t]{\textwidth}
\begin{tabular}{||M{1cm}|M{1cm}|M{1cm}|M{1.2cm}|M{1.3cm}|M{1.2cm}|M{1cm}|M{1cm}|M{1.15cm}|M{1cm}|M{1cm}||}
\hline
\multirow{2}{*}{Model} &\multicolumn{2}{|c|}{Quantity}&\multicolumn{2}{|c|}{Fluency}  &\multicolumn{3}{|c|}{Semantic Similarity (with test)}&\multicolumn{3}{|c|}{Syntactic Similarity (with train)}\\
\cline{2-11}
& Unique & Vocab & Grammar & Plausibility & Precision & Recall & F1 & Precision & Recall & F1\\
\hline \hline

Train&31650&9552&0.15&NA&0.78&0.781&0.781&NA&NA&NA\\
\hline
Test&3956&621&0.16&4.5&NA&NA&NA&0.609&0.609&0.609\\
\hline

%CVAE&35.7\%&0&\textbf{0.05}&\textbf{2.4}&0.796&0.755&0.775&0.657&0.62&0.638\\
%\hline


EDA&93.2\%&3480&0.22&5.7&
0.756 &	0.75	&0.753&	0.85&	0.85&	0.85\\
MM&94.6\%&0&0.14&3.76&0.773&\textbf{0.778}&0.776&0.601&0.602&0.602\\
\hline
VAE&29.8\%&0&0.07&2.61&\textbf{0.808}&0.764&\textbf{0.785}&0.648&0.616&0.632\\
\hline
GPT-2&\textbf{98.2}\%&\textbf{17386}&0.15&4.8
&0.77&0.774&0.772&\textbf{0.598}&\textbf{0.602}&\textbf{0.6}\\

\hline
\hline
\end{tabular}
\caption{Amazon }
\label{tab:phone}
\end{subtable}

==> fig_and_tables/results.tex <==

% #############result table 1 #############
\begin{table*}[t]
\small
\begin{center}
\begin{subtable}[t]{\textwidth}
\begin{tabular}{||M{1cm}|M{1cm}|M{1cm}|M{1.2cm}|M{1.3cm}|M{1.2cm}|M{1cm}|M{1cm}|M{1.15cm}|M{1cm}|M{1cm}||}
\hline
\multirow{2}{*}{Model} &\multicolumn{2}{|c|}{Quantity}&\multicolumn{2}{|c|}{Plausibility}  &\multicolumn{3}{|c|}{Semantic Similarity (with test)}&\multicolumn{3}{|c|}{Syntactic Similarity (with train)}\\
\cline{2-11}
& Unique & Vocab & Grammar & Perplexity & Precision & Recall & F1 & Precision & Recall & F1\\
\hline \hline

Train&31650&9552&0.15&NA&0.78&0.781&0.781&NA&NA&NA\\
\hline
Test&3956&621&0.16&4.5&NA&NA&NA&0.609&0.609&0.609\\
\hline
VAE&29.8\%&0&0.07&2.61&\textbf{0.808}&0.764&\textbf{0.785}&0.648&0.616&0.632\\
\hline
CVAE&35.7\%&0&\textbf{0.05}&\textbf{2.4}&0.796&0.755&0.775&0.657&0.62&0.638\\
\hline
MM&94.6\%&0&0.14&3.76&0.773&\textbf{0.778}&0.776&0.601&0.602&0.602\\
\hline
GPT-2&\textbf{98.2}\%&\textbf{17386}&0.15&4.8
&0.77&0.774&0.772&\textbf{0.598}&\textbf{0.602}&\textbf{0.6}\\
\hline
EDA&93.2\%&3480&0.22&5.7&
0.756 &	0.75	&0.753&	0.85&	0.85&	0.85\\
\hline
\end{tabular}
\caption{Amazon }
\label{tab:phone}
\end{subtable}

% #############result table 2 #############
\bigskip
\begin{subtable}[t]{\textwidth}
\begin{tabular}{||M{1cm}|M{1cm}|M{1cm}|M{1.2cm}|M{1.3cm}|M{1.2cm}|M{1cm}|M{1cm}|M{1.15cm}|M{1cm}|M{1cm}||}
\hline
\multirow{2}{*}{Model} &\multicolumn{2}{|c|}{Quantity}&\multicolumn{2}{|c|}{Plausibility}  &\multicolumn{3}{|c|}{Semantic Similarity (with test)}&\multicolumn{3}{|c|}{Syntactic Similarity (with train)}\\
\cline{2-11}
&Unique& Vocab&Grammar& Perplexity & Precision & Recall & F1& Precision & Recall & F1\\
\hline \hline
Train&24523&16211&0.060&NA&0.808&0.808&0.808&NA&NA&NA\\
\hline
Test&3065&850&0.058&6.36&NA&NA&NA&0.564&0.565&0.564\\
\hline
VAE&6.3\%&0&\textbf{0.017}&6.20&0.811&0.777&0.794&0.594&\textbf{0.555}&0.574\\
\hline
CVAE&65.8\%&0&0.023&\textbf{4.49}&\textbf{0.818}&0.799&\textbf{0.80}8&0.598&0.575&0.586\\
\hline
MM&92.9\%&0&0.056&4.54&0.806&\textbf{0.805}&0.805&0.568&0.569&0.568\\
\hline
GPT-2&\textbf{99.6}\%&\textbf{39104}&0.082&7.57&0.79&0.801&0.796&\textbf{0.556}&0.56&\textbf{0.558}\\
\hline
EDA&94.6\%&5405&0.258&13.688&0.612&0.606&0.609&0.842&0.842&0.842\\
\hline
\end{tabular}
\caption{News }
\label{tab:news}
\end{subtable}
\bigskip

% #############result table 3 #############

\begin{subtable}[t]{\textwidth}
\begin{tabular}{||M{1cm}|M{1cm}|M{1cm}|M{1.2cm}|M{1.3cm}|M{1.2cm}|M{1cm}|M{1cm}|M{1.15cm}|M{1cm}|M{1cm}||}
\hline
\multirow{2}{*}{Model} &\multicolumn{2}{|c|}{Quantity}&\multicolumn{2}{|c|}{Plausibility}  &\multicolumn{3}{|c|}{Semantic Similarity (with test)}&\multicolumn{3}{|c|}{Syntactic Similarity (with train)}\\
\cline{2-11}
&Unique& Vocab&Grammar& Perplexity & Precision & Recall & F1& Precision & Recall & F1\\
\hline \hline
Train &7015&6731&0.108&NA&0.79&0.785&0.787&NA&NA&NA\\ \hline
Test &871&431&0.106&5.10&NA&NA&NA&0.662&0.656&0.659\\ \hline
VAE &1.1\%&0&0.117&\textbf{1.61}&\textbf{0.787}&0.739&0.763&0.736&\textbf{0.637}&0.683\\ \hline
CVAE &12.9\%&0&0.117&2.43&0.78&0.759&0.769&0.706&0.668&0.687\\ \hline
MM &65.6\%&0&\textbf{0.089}&3.40&0.785&\textbf{0.782}&\textbf{0.784}&\textbf{0.649}&0.657&0.653\\ \hline
GPT-2 &\textbf{91.5}\%&\textbf{24816}&0.103&5.13&0.771&0.782&0.776&0.65&0.654&\textbf{0.652}\\ \hline
EDA &84.0\%&5467&0.205&5.46&0.743&0.749&0.746&0.85&0.851&0.851\\ \hline
\end{tabular}
\caption{Yahoo }
\label{tab:yahoo}
\end{subtable}
\end{center}
\caption{Corpora results}
\label{tab:results}
\end{table*}
